Reactive and human-in-the-loop planning and control of multi-robot systems under LTL specifications in dynamic environments

This paper investigates the planning and control problems for multi-robot systems under linear temporal logic (LTL) specifications. In contrast to most of existing literature, which presumes a static and known environment, our study focuses on dynamic environments that can have unknown moving obstacles like humans walking through. Depending on whether local communication is allowed between robots, we consider two different online re-planning approaches. When local communication is allowed, we propose a local trajectory generation algorithm for each robot to resolve conflicts that are detected on-line. In the other case, i.e., no communication is allowed, we develop a model predictive controller to reactively avoid potential collisions. In both cases, task satisfaction is guaranteed whenever it is feasible. In addition, we consider the human-in-the-loop scenario where humans may additionally take control of one or multiple robots. We design a mixed initiative controller for each robot to prevent unsafe human behaviors while guarantee the LTL satisfaction. Using our previous developed ROS software package, several experiments are conducted to demonstrate the effectiveness and the applicability of the proposed strategies.

==> settings.tex <==
\usepackage[
	citestyle=ieee, 
    bibstyle=ieee,
    style=numeric-comp,
    sorting=nty,
    maxbibnames=99, % Make sure we are printing all authors in the appendix
    ]{biblatex}
    
% Makes the last name first in the bibliography.
% \DeclareNameAlias{author}{last-first}
\DeclareNameAlias{author}{family-given}
    
% Specify the margins. This is 6.25inches in text with which 
% can be used to size figures to the correct size.
\usepackage[a4paper, margin=2.5625cm]{geometry}

\usepackage{eso-pic}					% Packages for layout and graphics 
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{fadings}
\usepackage{setspace}
% \usepackage{tocloft}		 			% Fixing a bug with page style changes for toc
% \tocloftpagestyle{plain}
\usepackage{etoc} 						% Separate tocs for appendix and the rest    
\usepackage{chngcntr}					% Count figures within chapters
\usepackage{booktabs}					% Table formatting
\usepackage{fancyhdr}					% Setting the style for header and footer.
\usepackage{tabularx}
\usepackage{multirow}                   % For better tables 
\usepackage[hidelinks]{hyperref}		% Clickable links
\usepackage{nameref}					% References with names
\usepackage[parfill]{parskip}			% New line instead of indent for sections
\usepackage{tcolorbox}					% Create boxes around content
\tcbset{colback=white,arc=0mm}

\usepackage[english]{babel}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathdots}
\usepackage{yhmath}
\usepackage{siunitx}
\usepackage{array}
\usepackage{gensymb}
\usepackage{amssymb}
\usepackage{mathtools}  

% New packages
%\usepackage[table]{xcolor}
%\usepackage{array}
%\usepackage{makecell}
%\usepackage{subcaption}
%\usepackage{placeins}


% Add text to math arrows.

\usepackage{cancel}
\usepackage{color}
\usepackage{multirow}
\usepackage{textcomp}               % Fixing warning for gensyb \perthousand
\usepackage{svg}                    % including svg files
\usepackage{caption}                % For subfigures
\usepackage{subcaption}
%\usepackage{fontspec}
\usepackage{sectsty}
\usepackage{tocloft}

\usepackage[printonlyused]{acronym}


\counterwithin{figure}{section} 
\counterwithin{table}{section}

% % Specifying fonts
% \setmainfont{Georgia} 
% \setsansfont{Arial}
% \newfontfamily\footerfont{Georgia}

\chapterfont{\sffamily\fontsize{17}{17}}
\sectionfont{\sffamily\fontsize{14}{15}}
\subsectionfont{\sffamily\fontsize{13}{15}}
\subsubsectionfont{\sffamily\fontsize{12}{15}}

% Remove the title and make sure that the text is adjusted
% \usepackage{abstract}
% \setlength{\absleftindent}{0mm}
% \renewcommand{\abstractname}{\vspace{-\baselineskip}}
% \renewcommand{\abstractnamefont}{\sffamily\fontsize{14}{15}}
% \renewcommand{\abstracttextfont}{\normalfont\fontsize{12}{13}}

% Renaming and setting style of table of contents
\renewcommand*\contentsname{Contents}
\renewcommand*\cfttoctitlefont{\fontsize{16}{0}\bf\sffamily}
\renewcommand\cftchapfont{\fontsize{14}{0}\bf\sffamily}
\renewcommand\cftchappagefont{\fontsize{13}{0}\bf\sffamily}
\renewcommand\cftsecfont{\fontsize{12}{0}\sffamily}
\renewcommand\cftsecpagefont{\fontsize{12}{0}\sffamily}
\renewcommand\cftsubsecfont{\fontsize{12}{0}\sffamily}
\renewcommand\cftsubsecpagefont{\fontsize{12}{0}\sffamily}

% Styling the header and footer
\fancyhf{}
\fancyhead{}
\fancyfoot{}
\fancyhead[L]{\fontsize{11}{10}\selectfont\leftmark}
\fancyfoot[R]{\footerfont\thepage}
\setlength{\headheight}{15.5pt}


\fancypagestyle{plain}{
    \fancyhf{}
    \fancyhead{}
    \fancyfoot{}
    \renewcommand{\headrulewidth}{0pt}
    \fancyfoot[R]{\footerfont\thepage}
}

\pagestyle{fancy}

% Making the command for placing text in random locations
\newcommand\PlaceText[3]{%
\begin{tikzpicture}[remember picture,overlay]
\node[outer sep=0pt,inner sep=0pt,anchor=south west] 
  at ([xshift=#1,yshift=-#2]current page.north west) {#3};
\end{tikzpicture}%
}

% Disable hyphenation
\pretolerance=10000
\tolerance=2000 
\emergencystretch=50pt

